PHOENIX: Device-Centric Cellular Network Protocol Monitoring using Runtime Verification

End-user-devices in the current cellular ecosystem are prone to many different vulnerabilities across different generations and protocol layers. Fixing these vulnerabilities retrospectively can be expensive, challenging, or just infeasible. A pragmatic approach for dealing with such a diverse set of vulnerabilities would be to identify attack attempts at runtime on the device side, and thwart them with mitigating and corrective actions. Towards this goal, in the paper we propose a general and extendable approach called Phoenix for identifying n-day cellular network control-plane vulnerabilities as well as dangerous practices of network operators from the device vantage point. Phoenix monitors the device-side cellular network traffic for performing signature-based unexpected behavior detection through lightweight runtime verification techniques. Signatures in Phoenix can be manually-crafted by a cellular network security expert or can be automatically synthesized using an optional component of Phoenix, which reduces the signature synthesis problem to the language learning from the informant problem. Based on the corrective actions that are available to Phoenix when an undesired behavior is detected, different instantiations of Phoenix are possible: a full-fledged defense when deployed inside a baseband processor; a user warning system when deployed as a mobile application; a probe for identifying attacks in the wild. One such instantiation of Phoenix was able to identify all 15 representative n-day vulnerabilities and unsafe practices of 4G LTE networks considered in our evaluation with a high packet processing speed (~68000 packets/second) while inducing only a moderate amount of energy overhead (~4mW).

==> resources/lte-attack-signature-table.tex <==
\begin{table}[ht]
    \centering
\caption{PLTL FORMULAS GENERATED BY SIGNATURE SYNTHESIZER [SAT-Core].}
\label{table:eval-dataset-2}
%\rowcolors{1}{gray!25}{white}
%\makebox[\textwidth]{
\resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|}
        \hline
%        \rowcolor{gray!50}    
        \textbf{LTE Attacks}  & \textbf{Synthesized Sigantures [core-SAT]} & \textbf{Attack Behavior}\\ \hline
        Numb Attack           &  $\globally((\mathsf{authentication\_reject} \Rightarrow (\mathsf{authentication\_reject} \since\mathsf{authentication\_response})))$ & It is always the case that authentication response precedes authentication reject. \\ \hline
        Paging with IMSI      &  $\globally(\neg((\mathsf{paging\_IMSI\_and\_TMSI}\vee\mathsf{paging\_IMSI})))$ & It is always the case that no message is passed with IMSI or TMSI. \\ \hline
        Null Encryption       &  $\globally(\neg(\mathsf{MME\_null\_encryption\_chosen})))$ & Null encryption or null integrity are selected even if the UE supports other encryption algorithms.\\ \hline
        RLF Report            &  $\globally((\mathsf{ueInformationResponse\textnormal{-}r9}\Rightarrow((\mathsf{rrcConnectionRelease}\Rightarrow\mathsf{ueInformationResponse\textnormal{-}r9})\since\mathsf{securityModeComplete})))$ & ?\\ \hline
        RLF Report            &  $\globally((\mathsf{ueInformationResponse\textnormal{-}r9}\Rightarrow(\neg (ueCapabilityInformation) \since\mathsf{securityModeComplete})))$ & ?\\ \hline  
        RLF Report            &  $\globally((\mathsf{ueInformationResponse\textnormal{-}r9}\Rightarrow(\neg (ueCapabilityInformation) \since\mathsf{securityModeCommand})))$ & ?\\ \hline  
        RLF Report            &  $\globally((\mathsf{ueInformationResponse\textnormal{-}r9}\Rightarrow(\neg (ueCapabilityEnquiry) \since\mathsf{securityModeCommand})))$ & ?\\ \hline  
        Malformed Identity    & $\globally(\neg(\mathsf{identity\_request\_not\_well\_formed})))$ & ?\\ \hline
        IMSI Catching         &  $\globally(\neg(\mathsf{identity\_request\_IMSI})))$ & ?\\ \hline
        Measurement Report    &  None & None \\ \hline
        Aka Bypass            & $\globally((\mathsf{rrcConnectionReconfiguration}\Rightarrow((\mathsf{rrcConnectionRequest}\Rightarrow\mathsf{securityModeComplete})\since\mathsf{securityModeComplete})))$ & ?\\ \hline
        Aka Bypass            & $\globally((\mathsf{rrcConnectionReconfiguration}\Rightarrow(\neg(\mathsf{rrcConnectionRelease})\since\mathsf{securityModeCommand})))$ & RRC Connection reconfiguration occurs before security mode command procedure. \\ \hline
        IMSI Cracking         &  $\globally(\neg(\mathsf{paging\_IMSI\_and\_TMSI})))$ & No paging with IMSI/TMSI. \\ \hline
    \end{tabular}        
    }
\end{table}



==> resources/pltl-example.tex <==
\begin{example}
For a better understanding of how \pltl represents a vulnerability signature, let us consider 
the following  measurement report attack signature $\Phi$:
%
\begin{equation*}
\resizebox{.99\columnwidth}{!}{$\measurementReport \Rightarrow \yesterday (\neg \rrcConnectionRequest \since \securityModeComplete)$}
\end{equation*}
%
This vulnerability signature states that if there is a \textsf{measurement report} message sent by the UE then it is not the case
that UE has started a new session (i.e., sent an \rrcConnectionRequest message)
 since the last time a security context was established (i.e., sent a \securityModeComplete message).
%\[
%\Phi = 
%\measurementReport \Rightarrow \yesterday (\neg \rrcConnectionRequest \since \securityModeComplete)
%\]
%
%
In Table~\ref{table:attk-eg}, we show evaluation 
of this vulnerability signature $\Phi$ using few example positive (benign) and 
negative (malicious) traces.
%
We can see that the vulnerability signature $\Phi$ is only falsified for an attack trace and 
remains true for all positive traces that exhibit benign traffic. 
%
Thus, a monitor built using $\Phi$ correctly alarms the user about the occurrence of measurement report attack behavior. 
%
\begin{table}[]
    \centering
\resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{|c|c|l|l|l|}
        \hline
        & &\measurementReport & \rrcConnectionRequest &  \securityModeComplete \\
        \hline
        $\sigma$ & $\Phi$ & $\sigma_{0}\sigma_{1}\sigma_{2}\sigma_{3}$ & $\sigma_{0}\sigma_{1}\sigma_{2}\sigma_{3}$ & $\sigma_{0}\sigma_{1}\sigma_{2}\sigma_{3}$ \\       
        \hline
        P1&\true & \texttt{0000} & \texttt{0100} & \texttt{1000} \\
        P2&\true & \texttt{0110} & \texttt{0100} & \texttt{1101}\\
        P3&\true & \texttt{0011} & \texttt{0110} & \texttt{0110} \\ \hline
        N4&\false & \texttt{1011} & \texttt{0110} & \texttt{1001}\\
        N5&\false & \texttt{1001} & \texttt{0100} & \texttt{1001}\\
        N6&\false & \texttt{0001} & \texttt{0110} & \texttt{0001}\\
        \hline      
        \end{tabular}    
}
\caption{$\Phi$ over positive traces [P1-P3] and negative traces [N4-N6].}
\label{table:attk-eg}
\end{table}

\end{example} 

